VarBench: Robust Language Model Benchmarking Through Dynamic Variable Perturbation

As large language models achieve impressive scores on traditional benchmarks, an increasing number of researchers are becoming concerned about benchmark data leakage during pre-training, commonly known as the data contamination problem. To ensure fair evaluation, recent benchmarks release only the training and validation sets, keeping the test set labels closed-source. They require anyone wishing to evaluate his language model to submit the model's predictions for centralized processing and then publish the model's result on their leaderboard. However, this submission process is inefficient and prevents effective error analysis. To address this issue, we propose to variabilize benchmarks and evaluate language models dynamically. Specifically, we extract variables from each test case and define a value range for each variable. For each evaluation, we sample new values from these value ranges to create unique test cases, thus ensuring a fresh evaluation each time. We applied this variable perturbation method to four datasets: GSM8K, ARC, CommonsenseQA, and TruthfulQA, which cover mathematical generation and multiple-choice tasks. Our experimental results demonstrate that this approach provides a more accurate assessment of the true capabilities of language models, effectively mitigating the contamination problem.

==> scrapwork.tex <==
\begin{table*}[t]
\centering
% \begin{adjustbox}{width=1.0\columnwidth,center}
\begin{tabular}{@{}lllccc@{}}
\toprule
LLM & Examples & Prompt & GSM-8K $\uparrow$ & GSM+ $\uparrow$ & $\Delta$ \\ \midrule
Yi-1.5 6B & 5 & Standard & 52.62 & 22.71 & 29.91 \\
Yi-1.5 6B & 8 & Chain-of-Thought & 61.33 & 27.51 & 33.82\\
Yi-1.5 9B & 5 & Standard & 66.11 & 28.40 & 37.71 \\
Yi-1.5 9B & 8 & Chain-of-Thought & 65.96 & 30.91 & 35.05 \\
\hline
Zephyr-7B $\beta$ & 5 & Standard & 33.43 & 15.86 & 17.57 \\
Zephyr-7B $\beta$ & 8 & Chain-of-Thought & 41.55 & 18.80 & 22.75 \\
Zephyr-7B $\gamma$ & 5 & Standard & 44.88 & 19.37 & 25.51 \\
Zephyr-7B $\gamma$ & 8 & Chain-of-Thought & 39.35 & 16.36 & 22.99\\
\hline
SeaLLM 2.5 7B & 5 & Standard & 75.28 & 33.35 & 41.93 \\
SeaLLM 2.5 7B & 8 & Chain-of-Thought & 75.66 & 34.64 & 41.02\\
\hline
DeepSeek Math Base 7B & 5 & Standard & 60.80 & 26.12 & 34.68 \\
DeepSeek Math Base 7B & 8 & Chain-of-Thought & 64.06 & 27.85 & 36.21 \\
DeepSeek Math Instruct 7B & 5 & Standard & 25.17 & 12.56 & 12.61 \\
DeepSeek Math Instruct 7B & 8 & Chain-of-Thought & 66.03 & 32.17 & 33.86\\
\hline
Gemma 7B & 5 & Standard & 52.01 & 23.66 & 28.35 \\
Gemma 7B & 8 & Chain-of-Thought & 55.72 & 23.90 & 31.82\\
Gemma 1.1 IT 7B & 5 & Standard & 51.33 & 22.70 & 28.63\\
Gemma 1.1 IT 7B & 8 & Chain-of-Thought & 47.99 & 22.11 & 25.87 \\
\hline
Llama 3 8B & 5 & Standard & 50.87 & 21.16 & 29.71\\
Llama 3 8B & 8 & Chain-of-Thought & 55.19 & 26.13 & 29.06 \\
Llama 3 Instruct 8B & 5 & Standard & 75.82 & 32.91 & 42.91 \\
Llama 3 Instruct 8B & 8 & Chain-of-Thought & 77.48 & 35.48 & 42.00 \\
\hline
Mistral v0.3 7B & 5 & Standard & 36.32 & 15.88 & 20.44\\
Mistral v0.3 7B & 8 & Chain-of-Thought & 40.18 & 17.64 & 22.54\\
Mistral v0.2 Instruct 7B & 5 & Standard & 42.23 & 18.55 & 23.68\\
Mistral v0.2 Instruct 7B & 8 & Chain-of-Thought & 42.61 & 18.27 & 24.34\\
\hline
% Phi 3 Mini-4K Instruct & 5 & Standard & 78.01 & 35.63 & 42.38 \\
% \hline
OpenChat 3.5 Gemma & 5 & Standard & 74.45 & 33.81  & 40.64 \\
OpenChat 3.5 Gemma & 8 & Chain-of-Thought & 75.74 & 34.09  & 41.65 \\
\hline
GPT 3.5 Turbo-0125 & 5 & Standard & 74.83 & 36.01 & 38.82 \\
GPT 3.5 Turbo-0125 & 8 & Chain-of-Thought & 76.04 & 35.85 & 40.19 \\
\hline
GPT 4 Turbo & 5 & Standard & 89.23 & 40.76 & 48.47 \\
GPT 4 Turbo & 8 & Chain-of-Thought & 81.27 & 38.34 & 42.92 \\
\hline
\bottomrule
\end{tabular}
\caption{
\textbf{Comparison of performance of various LLMs and prompting strategies on GSM8K and GSM8K+}. 
\label{tab:gsm8k_results}
}
% \end{adjustbox}
% \vspace{-2mm}
\end{table*}
